An Input-to-State Stability Perspective on Robust Locomotion

Uneven terrain necessarily transforms periodic walking into a non-periodic motion. As such, traditional stability analysis tools no longer adequately capture the ability of a bipedal robot to locomote in the presence of such disturbances. This motivates the need for analytical tools aimed at generalized notions of stability -- robustness. Towards this, we propose a novel definition of robustness, termed \emph{$\delta$-robustness}, to characterize the domain on which a nominal periodic orbit remains stable despite uncertain terrain. This definition is derived by treating perturbations in ground height as disturbances in the context of the input-to-state-stability (ISS) of the extended Poincar\'{e} map associated with a periodic orbit. The main theoretic result is the formulation of robust Lyapunov functions that certify $\delta$-robustness of periodic orbits. This yields an optimization framework for verifying $\delta$-robustness, which is demonstrated in simulation with a bipedal robot walking on uneven terrain.

==> Old_Sections/BarrierVerification_old.tex <==
\newpage 
\newsec{Barrier functions for $\delta$-robustness}
Consider again the discrete-time dynamical system defined in \eqref{eq: discretetime}: $x_{k+1} = P_{d_k}(x_k)$.   
Since the specific guard condition $d_k$ assigned to step $k$ is unknown, we will use a set-based Poincar\'e map to denote the collection of Poincar\'e return maps for all guard conditions contained within the set $\B_{\delta}(x^*)$:
\begin{align}
    \P_{\delta}(x) := \{P_d(x) \mid \forall d \in [d^-_{\delta},d^+_{\delta}]\}.
\end{align}
Thus, the discrete-time dynamical system for any guard condition $S_d$ with $d \in [d^-_{\delta},d^+_{\delta}]$ is denoted as the expanding set:
\begin{align}
    \bm{X}_{k+1} := \P_{\delta}(x_k).
    \label{eq: setDiscrete}
\end{align}

Using this set-based notion of a discrete-time dynamical system, we propose the following theorem:
\begin{theorem}
    Consider the discrete-time barrier function, $H_{\delta}: \X \to \R$, defined as $H_{\delta}(x):= \delta^2 - \|x - x^*\|^2 \geq 0$. If the following condition is satisfied: 
    $$\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0), \quad \gamma \in (0,1],$$
    for all $x_0 \in \B_{\delta}(x^*)$, then the periodic orbit $\O$ is $\delta$-robust.
\end{theorem}
\begin{proof}
     Given some $\delta > 0$, with corresponding $\{d^-_{\delta},d^+_{\delta}\} \in \R$ per Definition \ref{def: deltarobust}, then the set $\B_{\delta}(x^*)$ is a 0-superlevel set of the continuously differentiable function $H_{\delta}: \X \to \R$ satisfying: 
    \begin{align*}
        \B_{\delta}(x^*) := \{x \in \X \mid H_{\delta}(x) \geq 0\} \\
        \partial \B_{\delta}(x^*) := \{x \in \X \mid H_{\delta}(x) = 0 \}
    \end{align*}
    
    Per Proposition 4 of \cite{agrawal2017discrete}, the discrete-time system \eqref{eq: discretetime}, for a specific choice of $d_k \in [d^-_{\delta},d^+_{\delta}]$, is forward-set invariant with respect to the set $\B_{\delta}(x^*)$ if $H_{\delta}$ satisfies the following conditions for all $x_0 \in \B_{\delta}(x^*)$:
    \begin{enumerate}
        \item $H_\delta(x_0) \geq 0$,
        \item $H_{\delta}(P_{d_k}(x_k))-H_{\delta}(x_k) \geq -\gamma H_{\delta}(x_k)$, \\$\forall k \in \mathbb{Z}^+$, $0 < \gamma \leq 1$,
    \end{enumerate}
    where the second condition can be rewritten as $H_{\delta}(P_{d_k}(x_k)) \geq (1-\gamma) H_{\delta}(x_k)$.

    Using Lemma \ref{lemma: recursiveset}, $P_{d_k}(x_k) \in \B_{\delta}(x^*)$ for all $k \in \mathbb{Z}^+$ if $P_{d_k}(x_0) \in \B_{\delta}$ for all $x_0 \in \B_{\delta}(x^*)$. Thus, we only need to check the second condition for some set $x_0 \in \B_{\delta}(x^*)$:
    $$H_{\delta}(P_{d_k}(x_0)) \geq (1-\gamma)H_{\delta}(x_0), ~0 < \gamma \leq 1.$$ Lastly, the above condition can be checked for all $d_k \in [d^-_{\delta},d^+_{\delta}]$ by ensuring that the smallest condition $$\min_{d \in [d^-_{\delta},d^+_{\delta}]}\{H_{\delta}(P_{d}(x))\} \geq (1-\gamma)H_\delta(x), $$ is satisfied. 
    Thus, the condition $$\min \{H_{\delta}(\bm{X}_{k})\} \geq (1-\gamma)H_{\delta}(x_0), \quad \gamma \in (0,1],$$ for all $x_0 \in \B_{\delta}(x^*)$ enforces that 
    $\bm{X}_{k+1} = \P_{\delta}(x_k)$ is forward set invariant with respect to the set $\B_{\delta}(x^*)$. This is equivalent to the statement that $ P_d(\B_{\delta}(x^*)) \subseteq \B_{\delta}(x^*), ~\forall d \in [d^-_{\delta},d^+_{\delta}]$. Therefore, per Definition \ref{def: deltarobust}, $\O$ is $\delta$-robust to $d \in [d^-_{\delta},d^+_{\delta}]$.
\end{proof}

% \begin{theorem}
%     If $ H_{\delta}(P_{d_k}(x_k)) \geq \gamma H_{\delta}(x_k)$ for all $x_k \in \B_{\delta}(x^*)$, then $\O$ is $\delta$-robust and the discrete-time system \eqref{eq: discretetime} is exponentially stable.
% \end{theorem}
% \begin{proof}
%     \red{?}
% \end{proof}


% We can use sample-based approach:
% \begin{enumerate}
%     \item Starting with a small $\delta > 0$, fix $\delta > 0$ and sample the boundary of $\B_{\delta}(x^*)$ (i.e. $s_i \sim \partial \B_{\delta}(x^*))$)
%     \item Observe the flow $\varphi_t(\Delta(s_i))$ $\forall s_i \in samples$
%     \item The set-valued Poincar\'e map is equal to a portion of this flow: $$ \P_{[d^-,d^+]}:=\{ \varphi_t(\Delta(s_i)) \mid t \in [T_e(\Delta(s_i),d^+),T_e(\Delta(s_i),d^-)]\}$$ \red{Note: This currently assumes that $\dot{h}<0$ for $h \in [d^-,d^+]$}
%     \item If $\P_{[d^-,d^+]}(s_i) \in \B_{\delta}(x^*)$ for the selected $\delta > 0$, then increase $\delta$ and repeat the process. If not, then the orbit $\O$ is $\delta$-robust to $d \in [d^-,d^+]$.
% \end{enumerate}

\newsubsec{Probablistic Verification Approach}
It is important to recognize that verifying the condition $\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0)$ for all $x_0 \in \B_{\delta}(x^*)$ is computationally infeasible. This is especially true for systems in which the Poincar\'e map is not available explicitly. Thus, we will instead use sampling methods to verify $\delta$-robustness with probabilistic guarantees. 

% Mainly, we will transform the problem into the following uncertain program:
% \begin{align}
%     \delta^* = &\argmax_{\delta > 0} \delta \\
%     &\text{s.t. } H_{\delta}(P_{d_k}(x_k)) \geq H_{\delta}(x_k), ~ 
% \end{align}

As outlined in \cite{akella2022barrier}, the certification of barrier functions can be probabilistic verified using sampling methods. First, we will introduce the method for verifying that a given periodic orbit is $\delta$-robust, for a given $\delta$. This algorithm is provided in Algorithm \ref{alg: givendelta}, and is outlined as follows.

\begin{algorithm}[tb]
\caption{Probabilistic Verification of Lemma 1}\label{alg: givendelta}
\begin{algorithmic}[1]
\Procedure{Given $\delta > 0$}{}
% {$\delta > 0$, $d^-_{\delta} := \inf\{h(x) \mid \B_{\delta}(x^*)\}$, $d^+_{\delta} := \sup\{h(x) \mid \B_{\delta}(x^*)\}$}
\State $x' \sim U(\B_{\delta}(x^*))$
\State Forward simulate $\P_{\delta}(x') \rightarrow \bm{X}_{1}$
\If {$\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0)$, $0 < \gamma \leq 1$} 
  \State $r_i = 1$
\Else
    \State $r_i = 0$
\EndIf 
\State Repeat sampling $r_i \to \{r_j\}^N_{j=1}$
\State Find minimum $r_j \to r^*_N$
\State Compute $\Prob_{\pi_r}^N[\Prob_{\pi_r}[r \geq r^*_N] \geq 1 - \varepsilon] \geq 1 - (1-\varepsilon)^N$
\EndProcedure
\end{algorithmic}
\end{algorithm}

%%% THIS SECTION NEEDS WORK
-----

Let $r$ be a random variable with an associated probability distribution $\pi_r$. To formalize this distribution, we define the indicator function $\bm{1}_x$


We can as such define the probability of sampling $r$ as the probability of sampling an initial condition $x \in \B_{\delta}(x^*)$ such that the corresponding set-valued Poincar\'e map $\P_{\delta}(x)$ is contained within the set $\B_{\delta}(x^*)$. As stated before, this condition is equivalent to the barrier function condition $\min \{H_{\delta}(\P_{\delta}(x))\} \geq (1-\gamma)H_{\delta}(x)$, for some $0 < \gamma \leq 1$.

In Algorithm \ref{alg: givendelta}, it is assumed that $\delta > 0$ is given. Then, by sampling $x' \in \B_{\delta}(x^*)$ with a uniform distribution over $\B_{\delta}(x^*)$, we can implicitly define the probability distribution function $\pi_r$ for the random variable $r$.

-----

To identify the largest $\delta > 0$ such that $\O$ is $\delta$-robust, consider the following optimization problem
\begin{align}
    \label{eq: optdelta}
    (\delta^*, \gamma^*) = &\argmax_{\delta > 0,\gamma \in (0,1]} \delta \\
    &\text{s.t. } \min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0) \notag \\
    & \quad \forall x_0 \in \B_{\delta}(x^*) \notag
\end{align}

Again, we can use sampling to probabilistically identify $\delta^*$ and $\gamma^*$ using Algorithm \ref{alg: maxdelta}.

\begin{algorithm}[tb]
\caption{Probabilistic Approach to \eqref{eq: optdelta}}\label{alg: maxdelta}
\begin{algorithmic}[1]
\Procedure{}{}
% {$\delta > 0$, $d^-_{\delta} := \inf\{h(x) \mid \B_{\delta}(x^*)\}$, $d^+_{\delta} := \sup\{h(x) \mid \B_{\delta}(x^*)\}$}
\State $\delta' \sim U(\Omega)$
\State Verify $r^*_N \geq 0$ given $\delta'$ using Alg. \ref{alg: givendelta}
\If {$r^*_N \geq 0$}
    \State Add $\delta'$ to $\{\delta_j\}^N_{j=1}$
\Else
    \State Reject $\delta'$
\EndIf
\State $\max\{\delta_j\}^N_{j=1} \rightarrow \delta^*_N$
\State Compute $\Prob_{\pi_{\delta}}^N[\Prob_{\pi_{\delta}}[\delta \leq \delta^*_N] \geq 1 - \varepsilon] \geq 1 - (1-\varepsilon)^N$
\EndProcedure
\end{algorithmic}
\end{algorithm}


%%%%% OLD STUFF!! 
% \subsection{Theoretical Guarantees using Stochastic Processes}

% The discrete-time dynamical system in the presence of uncertain impact events can be considered as a stochastic system:
% $$ x_{k+1} = P_d$$

% Our definition for Hybrid Set Invariant walking can now be extended to the following:
% \begin{definition} 
%     A hybrid system $\H\C$ with a periodic orbit $\O$ is defined as \textit{Robustly Hybrid Set Invariant} if there exists some set $\D := \{x^-_i \in S \oplus S_d \mid \forall d \in [-\gamma,\gamma]\}$ such that $P_d(x^-_i) \in \D$ for all $x^-_i \in \D$ and for all $d \in [-\gamma, \gamma]$. .
% \end{definition}

% \subsection{Proving that an orbit $\O$ is Robustly HSI}
% Let $H$ denote the trajectory of the guard condition $h(x)$ (in our case the vertical position of the swing foot relative to the stance foot) computed by:
% $$ H(x_0,d) := \{ h(\varphi_t(x_0) \mid 0 \leq t \leq T_{e}(x_0,d)\} \in \R.$$ 

% \begin{assumption}
%     We assume that for $x_0 = \Delta(x^*)$, there exists some $\{T_h,h_{\max}\} \in \R^+$ such that the flow of the system $\varphi_t(x_0)$ evolves such that:
%     \begin{small}
%     \begin{numcases}{}
%         h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) > 0 & $0 \leq t < T_h$, \notag \\
%         h(\varphi_t(x_0)) = h_{\max}, ~\dot{h}(\varphi_t(x_0)) = 0 & $t = T_h$, \notag  \\
%         h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) < 0 & $T_h < t < T_e(x_0,-\gamma)$, \notag \\
%         h(\varphi_t(x_0)) = -\gamma, ~\dot{h}(\varphi_t(x_0)) < 0 & $t = T_e(x_0,-\gamma)$. \notag
%     \end{numcases}
%     \end{small}
%     \label{assump: swingfoot}
% \end{assumption}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/swingfoot.pdf}
%     \caption{Example Swing Foot Trajectory Satisfying Assumption \ref{assump: swingfoot}.}
%     \label{fig: swingfootassump}
% \end{figure}

% \begin{lemma}
%     Let $H(x_0,-\gamma)$ be a trajectory of the continuous guard condition $h(x) \in \R$ that satisfies Assumption \ref{assump: swingfoot}. If $h_{\max} \geq \gamma$, then %if $h(\varphi_t(\Delta(x^*))) \in \R^+$ is monotonically decreasing for all $t \in [T_h, T_e(x_0,-\gamma)]$, and  then 
%     $$T_e(\Delta(x^*),\gamma) \leq T_e(\Delta(x^*),0) \leq T_e(\Delta(x^*),-\gamma).$$ 
%     \label{lemma: orderedtime}
% \end{lemma}
% \begin{proof}
%     Per assumption \ref{assump: swingfoot}, the evaluation of the guard condition is $h(\varphi_t(x_0)) = \{h_{\max},-\gamma\}$ for $t = \{T_h, T_e(x_0,-\gamma)\}$. Additionally, we know that $h(\varphi_t(x_0))$ is monotonically decreasing in the interval $t \in (T_h,T_e(x_0,-\gamma))$ due to the assumption that in this range, $\dot{h}(\varphi_t(x_0)) < 0$. Thus, by the intermediate value theorem, we know that there must exist some $\{T_e(x_0,\gamma),T_e(x_0,0)\} \in (T_h,T_e(x_0,-\gamma))$ such that $\{h(\varphi_{T_e(x_0,0)}(x_0)),h(\varphi_{T_e(x_0,\gamma)}(x_0)) \} \in (h(\varphi_{T_h}(x_0)), h(\varphi_{T_e(x_0,-\gamma)}(x_0)))$. Additionally, since $h$ is monotonically decreasing in $t \in (T_h,T_e(x_0,-\gamma))$, then $h(\varphi_t(x_0)) = \gamma$ will occur at time $T_e(x_0,\gamma)$ before the height will reach $h(\varphi_t(x_0)) = 0$ at time $T_e(x_0,0)$. Thus, $T_e(x_0,\gamma) \leq T_e(x_0,0) \leq T_e(\Delta(x^*),-\gamma)$. 
% \end{proof}

% For ease of notation, we will denote the flow of our system between the guards $S_{\gamma}$ and $S_{-\gamma}$ as:
% \begin{align}
%     \varphi^*_t(x_0) := \{ \varphi_t(x_0) \mid T_e(x_0,\gamma) \leq t \leq T_e(x_0,-\gamma) \}.
% \end{align}
% \begin{lemma}
%     Consider a periodic orbit $\O$ with a fixed point $x^* \in \S_0$ satisfying $P_{0,0}(x^*) = x^*$. Assuming that $H(x_0,-\gamma)$ satisfies the properties of Assumption \ref{assump: swingfoot} for $x_0 = \Delta(x^*)$ and enforcing $h_{\max} \geq \gamma$, then the following holds:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmax_{t \in R^+} \|\varphi^*_t(x_0) - x^*\|
%     \end{align}
% \end{lemma}
% \begin{proof}
% It is known that $h: \X \to \R$ is continuous with $\dot{h} < 0$ for $t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)]$. It is also known that the arguments of $h$ (i.e. $\varphi_t(x_0) \in \X$) are also continuous. Thus, since $\|\varphi^*_t(x_0) - x^*\| = 0$ lies in the interior of $t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)]$ (using the ordering of $T_e(x_0,\gamma) \leq T_e(x_0,0) \leq T_e(\Delta(x^*),-\gamma)$ from Lemma \ref{lemma: orderedtime}), then $h(x)$ must take its largest values at the boundary of the set ($t =\{T_e(x_0,\gamma),T_e(x_0,-\gamma)\}$).
% \end{proof}

% \red{Next, we will assume that the continuous-time flow of some periodic orbit $\O$ satisfies the following assumption. Note that we later prove that this assumption is true for certain bipedal systems.}
% \begin{assumption}
%     Assume that given a periodic orbit $\O$ with a fixed point $P_0(x^*) = x^*$, then $\varphi^*(\Delta(x^*))$ evolves such that for $x_0 := \Delta(x^*) \in \Delta(\S_0)$:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmax_{t \in R^+} \|\Delta(\varphi^*_t(x_0)) - \Delta(x^*)\|
%     \end{align}
%     \label{assumption: maxTreset}
% \end{assumption}

% \begin{lemma}
%     (For systems with one degree of underactuation) If the following is true: 
%     $$\{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmin_{t \in R^+} \|\Delta(\varphi^*_t(x_0)) - \Delta(x^*)\|, $$
%     then the following is also true:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmin_{t \in R^+} \|P_{i}(\varphi^*_t(x_0)) - x^*\|, \notag \\
%         ~\forall i \in [-\gamma, \gamma]
%     \end{align}
%     \label{lemma: maxTpointcare}
% \end{lemma}
% \begin{proof}
%     \red{? Need to make an argument about the flow $\varphi_t(x_0)$.... I think this also relies on the assumption that you have only one degree of underactuation plus some assumption about your closed loop system (maybe an ISS assumption about $\O$)}
% \end{proof}

% \begin{theorem}
%     Let $\O := \{\varphi_t(\Delta(x^*)) \mid 0 \leq t \leq T_e(\Delta(x^*),0) \}$ be a periodic orbit with a fixed point $x^*\in\S_0$ such that $P_{0,0}(x^*) = x^*$. Also, assume that $H(\Delta(x^*),-\gamma)$ satisfies Assumption \ref{assump: swingfoot}. Denote an early and late impact state associated with the flow $\varphi_t(\Delta(x^*))$ as:
%     \begin{align*}
%         x_e &:= \{\varphi_t(\Delta(x^*)) \in \X \mid t = T_e(\Delta(x^*),\gamma)\}, \\
%         x_l &:= \{\varphi_t(\Delta(x^*)) \in \X \mid t = T_e(\Delta(x^*),-\gamma)\}.
%     \end{align*}
%     Additionally, denote the Poincar\'e return map associated with the Poincar\'e sections $S_{\gamma}$ and $S_{-\gamma}$ as:
%     \begin{align*}
%         P_e(x) := \{ \varphi_{t}(\Delta(x)) \mid t = T_e(\Delta(x),\gamma) \}, \\
%         P_l(x) := \{ \varphi_{t}(\Delta(x)) \mid t = T_e(\Delta(x),-\gamma) \}
%     \end{align*}
%     The orbit $\O$ is \textit{Robustly Hybrid Set Invariant} for the set $\D := \textup{conv}(\{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\})$ if:
%     \begin{align*}
%         \varphi_t(x_0) \in \D, ~&\forall t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)], \\
%         &\forall x_0 \in \{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\}
%     \end{align*}
% \end{theorem}
% \begin{proof}
%     For $\D := \textup{conv}(\{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\})$, the orbit $\O$ is Robustly HSI if $P_d(x^-_i) \in \D$ for all $d \in [-\gamma,\gamma]$ and for all $x^-_i \in \D$.
%     Following Lemma \ref{lemma: maxTpointcare}, we know that the Poincar\'e map error is maximized for the flow $\varphi_t(x_0)$ evaluated at $t = \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\}$. Thus, it suffices to check the Poincar\'e return map of $x_e$ and $x_l$....
%     By ensuring that the flow $\varphi^*_t(x_0)$ remains within the convex hull of $\D$, then any point within the convex set must also return to $\D$. Thus, $P_d(\D) \in \D$ for any $d \in [-\gamma, \gamma]$.
%     % Furthermore, these pre-impact states will yield the largest subsequent error for the set of states $\D := \{P_e(x_e),P_e(x_l), P_l(x_e), P_l(x_l)\}$. Finally, 
% \end{proof}


==> Old_Sections/BipedExample.tex <==
\newpage
\section{Synthesizing a $\delta$-Robust Periodic Orbit for a Bipedal Robot}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/uncertain_guards3.pdf}
    \caption{\textbf{Illustration of Uncertain Guard Condition for Five-Link Walker.} The nominal level-ground guard conditions is shown on the left along with the configuration coordinates of the five-link walker model used in this work. In comparison, the proposed guard condition for uncertain terrain of height $\gamma$ at impact is illustrated on the right.}
    \label{fig: uncertainguard}
    \vspace{-2mm}
\end{figure}


\red{Through the construction of B\'ezier polynomials, we could ensure that the control points between $\{\varphi_{T_e(x_k,d^-)}(x_k), \varphi_{T_e(x_k,d^+)}(x_k) \}$ lie inside of $\B_{\delta}(x^*)$}

As described in \cite{grizzle2014models}, a bipedal robot is classically modeled as a tree structure composed of rigid links by constructing a floating-base Lagrangian model and adding holonomic constraints to enforce the ground contact forces. Towards this, we will denote the floating-base reference frame of the bipedal robot as $R_b := [p,\phi]^{\top}$ with $p \in \R^3$ denoting the Cartesian position of the body-fixed reference and $\phi \in SO(3)$ denoting the orientation with respect to the world frame. The generalized configuration coordinates of the robot are then denoted as:
$$ q := (p,\phi,q_b) \in \Q = R^3 \times SO(3) \times D_b,$$
with $q_b \in \R^n$ being the body coordinates, representing the positions of $n \in \Z^+$ actuated joints. The state of the system is then denoted by $x := [q,\dot{q}]^{\top} \in \Q \times T\Q = R^{2n}$.

Next, the continuous dynamics of the system can be obtained via the Euler-Lange equation and holonomic constraints:
\begin{align}
    D(q)\ddot{q} + H(q,\dot{q}) = Bu + J_h^{\top}(q)F,
    \label{eq: Euler-Lagrange}
\end{align} 
where $D: \R^n \to \R^{n \times n}$ is the inertia matrix, $H(q,\dot{q}) := C(q,\dot{q})\dot{q} + G(q)$ is the vector containing the Coriolis and Gravity terms, $B: \Q \to \R^n$ is the actuation matrix, $u \in \R^m$ is the control input, $J_h(q) := \frac{\partial \nu(q)}{\partial q} \in \R^{J \times n}$ is the Jacobian of the holonomic constraints with $\nu(q) \in \R^h$ being the $h \in \Z^+$ holonomic constraints (stance foot position for robot with point-foot contacts; stance foot position and orientation for robot with flat-foot contacts). Lastly, $F \in \R^h$ is the contact wrenches which can be computed by solving the second order derivative of the holonomic constraints,
\begin{align}
    J_h(q)\ddot{q} + \dot{J}_h(q,\dot{q})\ddot{q}) = 0,    
\end{align}
and \eqref{eq: Euler-Lagrange} simultaneously. Next, we derive an impact map, $\Delta(q,\dot{q}) := [\Delta_q(q), \Delta_{\dot{q}}(q,\dot{q})]^{\top}$ based on the rigid impact model from \cite{hurmuzlu1994rigid} and assuming that the impacting foot neither slips nor rotates. Explicitly, the impact map is derived using the following system of equations (as in (27) of \cite{glocker1992dynamical}):
\begin{align}
    \begin{bmatrix}D(q) & -J_h^{\top}(q) \\ J_h(q) & 0_{h \times h}\end{bmatrix}\begin{bmatrix}\dot{q}^+ \\ F\end{bmatrix} = \begin{bmatrix} D \dot{q}^- \\ 0_{h \times n} \end{bmatrix}
\end{align}
Solving for the post-impact velocity, the resulting impact map is:
\begin{align}
    x^+ := (q^+,\dot{q}^+)^{\top} = \Delta(q^-,\dot{q}^-) = \begin{bmatrix} \Delta_q(q^-) \\ \Delta_{\dot{q}}(q^-,\dot{q}^-)   \end{bmatrix} \\
    ~= \begin{bmatrix}
        R q^- \\ (R - R(D^{-1}J_h^{\top}(J_hD^{-1}J_h^{\top})^{-1}J_h))\dot{q}^-
    \end{bmatrix},
\end{align}
with the arguments of $D(Rq^-)$ and $J_h(Rq^-)$ suppressed for ease of notation, and with $R \in \R^{n \times n}$ denoting the relabeling matrix (if no relabeling is required then $R = I_{n \times n}$).

One method of synthesizing periodic orbits $\O$ for bipedal robots is using the method of \textit{(Partial) Hybrid Zero Dynamics} \cite{ames2014human, westervelt2003hybrid}. This methods synthesizes output-level trajectories (often referred to as \textit{gaits}) which describe the desired behavior of the actuated coordinates of the robot (termed virtual constraints) such that when these outputs are enforced, the full nonlinear dynamics are rendered stable even in the presence of underactuation and impact events. Specifically, the virtual constraints, $y: \Q \to \R^m$, are defined as:
$$ y(q,\alpha) = y^a(q) - y^d(\tau(q),\alpha),$$
with $y^a(q) \in \R^m$ being the actual measured outputs and $y^d(\tau(q),\alpha) \in \R^m$ being the desired output parameterized by a monotonically increasing phasing variable $\tau: \Q \to \R$. Note that we choose specifically to parameterize $y^d$ using $N^{\text{th}}$ order B\'ezier polynomials, parameterized by the B\'ezier coefficients $\alpha \in \R^{m \times N}$. Using this paramterization, the virtual constraints can be shaped to satisfy an impact-invariance condition and stable closed loop dynamics via the trajectory optimization problem (as in \cite{tucker2021preference}):
\begin{ruledtable}
\vspace{-2mm}
{\textbf{\normalsize Trajectory Optimization:}}
\par\vspace{-4mm}{\small 
\begin{align*} \label{eq:opt}
   \{\alpha^*,X^*\} = \argmin_{\alpha,X} &~  \Phi(X) \\
    \text{s.t.}\quad 
    & \dot{x} = f_{cl}(x) \tag{Closed-loop Dynamics} \\
    & \Delta(\mathcal{S} \cap \mathcal{Z}_\alpha) \subset \mathcal{Z}_\alpha \tag{HZD Condition} \\
    % & y+K_py+K_s\dot y = 0 \tag{Dynamics Condition} \\
    & X_{\text{min}}  \preceq X \preceq X_{\text{max}} \tag{Decision Variables} \\
    & c_{\text{min}}  \preceq c(X) \preceq c_{\text{max}} \tag{Physical Constraints} 
    \label{eq: essential} 
    % &\text{(C1)~}\text{hybrid dynamics} ~\eqref{eq:EOM} \notag\\
    % &\text{(C2)~}%\text{HZD condition} \notag\\ 
    %     y^- = \dot y^- = y^+ = \dot y^+ = 0 \notag\\ 
    % &\text{(C2)~} \red{y+K_p y+ K_d\dot y= 0} \notag \\
    % &\text{(C3)~} % \text{physical feasibility}
    %     \mathcal{F}(q, \dot{q}) \preceq 0 \quad \forall t \notag\\ 
    % &\text{(C4)~} \text{essential constraints}  \notag 
\end{align*}}\vspace{-6mm}\par
\end{ruledtable}
\noindent where $X = (x_0,...,x_C,T)$ is the collection of all decision variables with $x_i$ the state at the $i^{th}$ discretization and $T$ the duration, $\Phi(X)$ is the cost function, and $c(X)$ is the set of physical constraints on the optimization problem. These physical constraints are included in every gait generation framework to encode the physical laws of real-word, such as the friction cone condition, workspace limit, and motor capacity \cite{reher2020algorithmic}.

 
%%%  SWITCH IN TOPIC...?
% Under Assumption 2, there is a unique mapping between $h(q)$ and $\tau(q)$ for states such that $\dot{h} < 0$. We will denote this mapping as $\Omega: \R \to \R$, with $$\Omega(d) := \{\tau(q) \mid h(q) = d, \dot{h}(q) < 0\}.$$

% \begin{theorem}
%     A periodic orbit $\O$ corresponding to the virtual constraints $y(q,\alpha^*)$ is Robust HSI to uncertain ground heights $d \in [-\gamma,\gamma]$ if $y^d(\Omega(\gamma),\alpha^*)$ and $y^d(\Omega(-\gamma),\alpha^*)$ ... 
% \end{theorem}


% \begin{lemma}
%     Given a biped with either point-foot contacts, or with flat-foot contacts and a swing-foot controller enforcing that the foot remains flat throughout the swing phase, then Assumption \ref{assumption: maxTreset} is true if $\forall q \in \varphi^*_t(x_0)$:
%     \begin{align}
%         \frac{\partial^2 J_h(q)}{\partial q^2} > 0, \\
%         \frac{\partial^2 D(q)}{\partial q^2} > 0
%     \end{align}
% \end{lemma}
% \begin{proof}
    
% \end{proof}

%%%  HOW TO SYNTHESIZE GAIT!
Let $\gamma > 0$ denote the largest ground height disturbance. Also, assume that the periodic orbit $\O$ satisfies the following assumption:

\begin{assumption}
    We assume that for $x_0 = \Delta(x^*)$, there exists some $\{T_h,h_{\max}\} \in \R^+$ such that the flow of the system $\varphi_t(x_0)$ evolves such that:
    \begin{small}
    \begin{numcases}{}
        h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) > 0 & $0 \leq t < T_h$, \notag \\
        h(\varphi_t(x_0)) = h_{\max}, ~\dot{h}(\varphi_t(x_0)) = 0 & $t = T_h$, \notag  \\
        h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) < 0 & $T_h < t < T_e(x_0,-\gamma)$, \notag \\
        h(\varphi_t(x_0)) = -\gamma, ~\dot{h}(\varphi_t(x_0)) < 0 & $t = T_e(x_0,-\gamma)$. \notag
    \end{numcases}
    \end{small}
    \label{assump: swingfoot}
\end{assumption}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/swingfoot.pdf}
    \caption{Example Swing Foot Trajectory Satisfying Assumption \ref{assump: swingfoot}.}
    \label{fig: swingfootassump}
\end{figure}

Under this assumption, we can show that $\O$ is guaranteed to intersect the guard conditions $S_{\gamma},S_{-\gamma}$ while respecting ordered time-to-impacts: $T_e(\Delta(x^*),\gamma) \leq T_e(\Delta(x^*),0) \leq T_e(\Delta(x^*),-\gamma)$.

\begin{lemma}
    Let $H(x_0,-\gamma)$ be a trajectory of the continuous guard condition $h(x) \in \R$ that satisfies Assumption \ref{assump: swingfoot}. If $h_{\max} \geq \gamma$, then %if $h(\varphi_t(\Delta(x^*))) \in \R^+$ is monotonically decreasing for all $t \in [T_h, T_e(x_0,-\gamma)]$, and  then 
    $$T_e(\Delta(x^*),\gamma) \leq T_e(\Delta(x^*),0) \leq T_e(\Delta(x^*),-\gamma).$$ 
    \label{lemma: orderedtime}
\end{lemma}
\begin{proof}
    Per assumption \ref{assump: swingfoot}, the evaluation of the guard condition is $h(\varphi_t(x_0)) = \{h_{\max},-\gamma\}$ for $t = \{T_h, T_e(x_0,-\gamma)\}$. Additionally, we know that $h(\varphi_t(x_0))$ is monotonically decreasing in the interval $t \in (T_h,T_e(x_0,-\gamma))$ due to the assumption that in this range, $\dot{h}(\varphi_t(x_0)) < 0$. Thus, by the intermediate value theorem, we know that there must exist some $\{T_e(x_0,\gamma),T_e(x_0,0)\} \in (T_h,T_e(x_0,-\gamma))$ such that $\{h(\varphi_{T_e(x_0,0)}(x_0)),h(\varphi_{T_e(x_0,\gamma)}(x_0)) \} \in (h(\varphi_{T_h}(x_0)), h(\varphi_{T_e(x_0,-\gamma)}(x_0)))$. Additionally, since $h$ is monotonically decreasing in $t \in (T_h,T_e(x_0,-\gamma))$, then $h(\varphi_t(x_0)) = \gamma$ will occur at time $T_e(x_0,\gamma)$ before the height will reach $h(\varphi_t(x_0)) = 0$ at time $T_e(x_0,0)$. Thus, $T_e(x_0,\gamma) \leq T_e(x_0,0) \leq T_e(\Delta(x^*),-\gamma)$. 
\end{proof}

The disturbance to the pre-impact state caused by this guard uncertainty can be represented as:
\begin{align}
    P_{h_{\max}}(x) = P_0(x) + 
\end{align}

==> Old_Sections/Motivation.tex <==
\newpage
\section{Motivation for Set-Theoretic Perspective}
% Because of the ability to analyze the stability of periodic orbits, to date researchers have primarily described walking as a periodic orbits (or a family of periodic orbits). However, these tools breakdown when uncertain terrain and perturbations require the walking to be no longer be periodic. We will present an example to motivate this.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/motivation_figure.pdf}
    \caption{Demonstration of a periodic orbit with $\lambda_{\max}(\frac{\partial P}{\partial x} (x^*)) > 0$ (illustrated on the left) not being robust to variations in the guard condition (for this example, the ground height was increased by 1cm), while a periodic orbit with a larger $\lambda_{\max}$ (illustrated on the right) is comparatively more robust. This motivates the need for a set-theoretic perspective towards robustness of periodic orbits to uncertain guard conditions.}
    \label{fig: motivation}
\end{figure}

Practically, the stability of periodic orbits can be analyzed by evaluating the eigenvalues of the Poincar\'e return map linearized around the fixed point. Specifically, if the magnitude of the eigenvalues of $\frac{\partial P}{\partial x}(x^*)$ is less than one (i.e. $\lambda_{\max} \left (\frac{\partial P}{\partial x}(x^*)\right) < 1$), then the fixed point is stable \cite{perko2013differential,morris2005restricted,wendel2010rank}. 
% Note that in this process, the eigenvalues corresponding to states known to be nonperiodic, such as the horizontal position of the floating base frame. 
Since it is often difficult to compute the Poincar\'e map analytically, it is commonly numerically approximated. %by applying small perturbations to each state and forward simulating one step to obtain $P(x^*+\delta )$ which is then used to construct each row of the Jacobian successively.

% \begin{lemma}
%     Let $\O$ be a periodic orbit with fixed point $x^* \in S$. If $\lambda_{\max}(J_P) < 1$, then the $\O$ is contracting and stable.
% \end{lemma}
    
\begin{remark}
    Orbits $\O$ with lower $\lambda_{\max}$ are regarded as being \textit{more stable} than orbits with higher $\lambda_{\max}$ since they are more contractive around the fixed point.
\end{remark}

However, since the Poincar\'e map is evaluated at the fixed point, this notion of stability is only valid locally. This means that while this tool is useful for checking the stability of periodic orbits, it is no longer insightful for systems with uncertain guard events or disturbances that push the system away from the fixed point. 

\subsection{Simulation Example}
\blue{Take two gaits, with one gait having a smaller eigenvalues than the other. Show that in the presence of uncertain terrain, the "more stable gait" fails, while the other one doesn't.}

As illustrated in Figure \ref{fig: motivation}, the classic Poincar\'e analysis does not accurately reflect the robustness of periodic orbits to local disturbances in the guard condition. In this work, we will instead propose tools for discussing the stability of walking (described by either periodic and nonperiodic orbits) from a set-theoretic perspective. This will then allow us to introduce tools for analyzing the stability of walking away from the fixed point.



==> Old_Sections/SetTheory.tex <==
\newpage
\section{A Set Theoretic View of Walking}
To relax the requirement on periodicity for hybrid systems with impulse events, we instead will take a set theoretic perspective.

Consider a compact set of pre-impact states in the guard, $\D \subset S$, with each element of $\D$ being defined as $\D_i := x^-_i \in S$. Note that this set definition assumes a constant and fixed impact surface $S$ (we will relax this assumption in section \ref{sec: uncertainguard}). The corresponding post-impact states is denoted as $\Delta(\D)$. Using the continuity assumption on the impact map, we know since $\D$ is compact, $\Delta(\D)$ is also compact. Using this, we can define the set containing the continuous-time solutions to $\Delta(\D)$ as,
$$
\C := \{\varphi_t(\Delta(x^-_i)) \in \X\} \mid 0 \leq t \leq T_I(x^-_i), \forall x_i^- \in \D\}
$$

Taking the Poincar\'e map to again be the guard, and applying the Poincar\'e map \eqref{eq: poincare} to every point in our set, we can denote the set-based Poincar\'e map as $P(\D) := \{P(x^-_i) \mid \forall x^-_i \in \D\}$. Using this set-based Poincar\'e maps, we can determine stability of the discrete-time system \eqref{eq: discrete-system} through the following theorem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}
%     Let $P$ be the Poincar\'e map $P: S \to S$ applied to a hybrid system $\H\C$. The discrete-time system $$x^-_{k+1} = P(x^-_k)$$ is forward invariant w.r.t $\D$ for any $x_0 \in \D$ if and only if $P(\D) \subset \D$.
% \end{theorem}

% Thus, 
% \begin{definition}
%     A hybrid control system $\H\C$ is defined as \textit{hybrid set invariant} if $P(\D) \subset \D$.
% \end{definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
    A hybrid system $\H\C$ is defined as \textit{Hybrid Set Invariant} with respect to the set $\D \subset S$ if $P(\D) \subset \D$.
\end{definition}

\begin{theorem}
    A hybrid system $\H\C$ is Hybrid Set Invariant ($P(\D) \subset \D)$ if and only if the set of flows $\C := \{\varphi_t(\Delta(x^-_i) \mid 0 \leq t \leq T_I(x^-_i), \forall x^-_i \in \D\}$ is forward invariant and $\Delta(\C \cap S) \subset \C$.
\end{theorem}
\begin{proof}
    $(\Rightarrow)$ If $P(\D) \subset \D$, then by definition $\varphi_{T_I(x^-_i)}(\Delta(x^-_i)) \subset \D$. Thus, the set of all flows $\varphi_t(\Delta(x^-_i))$ must be forward invariant. Additionally, the impact map applied to initial conditions must be contained within this set of flows by construction of $\C$, a.k.a. $\varphi_0(\Delta(x^-_i)) = \Delta(x^-_i) \subset \C$ for all $x^-_i \in \D$. Thus, writing this in terms of the set, $\Delta(\D) \subset \C$. \\
    $(\Leftarrow)$ If $\C$ is forward invariant, then there must exist some set $\D := \{\C \cap S\}$ such that $\forall x_0 \in \C$, $\exists T \in \R^+$ s.t. $\varphi_T(x_0) \in \D$. Then, since $\Delta(\D) \subset \C$, the solution to the flow $\varphi_T(\Delta(\D)) \subset \D$. Thus, by definition of the Poincar\'e map, $P(\D) \subset \D$. 
\end{proof}

% Note that this definition is similar to the definition of \textit{hybrid invariance} as given in \cite{morris2009hybrid}, with the exception that \cite{morris2009hybrid} was in reference to a submanifold $\Z \subset \X$. Thus, the condition for hybrid invariance of $\Z$ in \cite{morris2009hybrid} was the condition $P(S \cap \Z) \subset S \cap \Z$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\blue{Definition 1 of \cite{morris2009hybrid} defined the following.}
\begin{definition}
    For an autonomous system with impulse effects, a submanifold $\Z \subset \X$ is \textit{forward invariant} if for each point $x \in \Z$, $f(x) \in T_x\Z$ where $T_x\Z$ is the tangent space of the manifold $\Z$ at point $x$. A submanifold $\Z$ is \textit{impact invariant} in an autonomous system with impulse effects, or in a control system with impulse effects, if for each point $x$ in $\S \cap \Z$, $\Delta(x) \in \Z$. A submanifold $\Z$ is \textit{hybrid invariant} if it is both forward invariant and impact invariant.
\end{definition}
Also from \cite{morris2009hybrid}, hybrid invariance of $\C$ is reflected in the Poincar\'e map as: $$P(\S \cap \C) \subset \S \cap \C$$. 
\end{comment}

Equipped with this set-based perspective on hybrid flows, we can determine the stability of the solution based on the stability of the set $\D$. Specifically, we propose the following theorem:
\begin{theorem}
    Let $\H\C$ denote a hybrid system with a certain guard condition $S$. If there exists a set $\D \subset S$ such that $P(\D) \subset \D$, then for any initial condition $x^-_0 \in \Delta(\D)$, the discrete-time system is stable as a set..?. \blue{The discrete-time system $z(k+1) = P(z(k))$ is stable if and only if there exists a set $\D$ such that $P(\D) \subset \D$.}
\end{theorem}
\begin{proof}
    \red{Not sure how to formally prove this since it seems almost too intuitive... aka if $P(\D) \subset \D$, then by definition it is forward set invariant.}
\end{proof}

\begin{comment}
\red{We could also come up with stable, asymptotically stable, and exponentially stable definitions for set stability... called something like ``Hybrid Set Stable'', ``Hybrid Set Asymptotically Stable'', and ``Hybrid Set Exponentially Stable''. Corresponding to the conditions $P(\D) \subseteq \D$, $P(\D) \subset \D$, and $P^i(\D) \subset \text{exp. shrinking set}$}
\end{comment}

Note that classic definitions of stability via periodicity still hold for the set-based perspective on stability.
\begin{corollary} 
If there exists a fixed point, defined by $P(x^*) = x^*$, then this still satisfies the conditions for set-based walking: $P(x^*) \subset x^*$. Therefore, stable periodic walking is sufficient for stable set-based walking. (Periodic walking is a subset of set-based walking).
\end{corollary}
\red{An interesting motivating example may be the compass gait biped, with convergence to a periodic orbit but nonperiodic behaviors in the beginning}

\begin{comment}
\subsection{Demonstration for Rabbit}
The domain of attraction for periodic orbits in the full dimensional model are difficult to estimate. However, Westervelt et al. have shown that domains of attraction for restricted Poincar\'e maps can be computed analytically. For example, in Section IV of \cite{westervelt2003hybrid}, the domain of attraction of the fixed point of the restricted Poincar\'e map, $\rho: S \cap \Z_{\alpha} \to S \cap \Z_{\alpha}$, was computed analytically for the RABBIT 5-link walker. 
\end{comment}

\subsection{Connections with Input to State Stability}
It is also interesting to note that the presentation of set-based walking is similar to input-to-state stable walking. Notably, the system $\dot{x} = f(x) + g(x)u$, is input to state stable (ISS) if there exists $\beta \in \KL$ and $\iota \in \K_{\infty}$ such that:
\begin{align}
    |\varphi_t(x_0)| \leq \beta(|x_0|,t) + \iota(\|u\|_{\infty}), ~ \forall x_0,u, ~ \forall t \geq 0.
\end{align}


Mainly, the interesting observation is the f ollowing lemma:

\begin{lemma}
    Given a hybrid periodic orbit that is Input to State Stable (ISS), the resulting system is also set-based stable.
\end{lemma}
\begin{proof}
    \red{From ISS we know that $\C$ is contained in a closed and bounded tube and we know that $P(\D) \subset \D$ for $\D := (\O \oplus \B_{\epsilon}(\O)) \cap S$.
    Note: Define ISS for Poincar\'e map (as discrete time system), then give conditions on CLFs to be ISS-CLFs.}
\end{proof}

==> Old_Sections/UncertainGuard.tex <==
\section{A Set Theoretic Perspective on Walking: $\delta$-Robustness}
\label{sec: uncertainguard}

This section provides the key formulation of robustness considered throughout this paper---that of $\delta$-robustness.  The core concept behind this definition is stability in and of itself is not a sufficiently rich concept to capture robustness, since it is purely local.  Thus, we define a set-theoretic notion of robustness leveraging the Poincar\'e map. 


\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/uncertain_guards3.pdf}
    \caption{Illustration of Uncertain Guard Condition for Five-Link Walker. The nominal level-ground guard conditions is shown on the left along with the configuration coordinates of the five-link walker model used in this work. In comparison, the proposed guard condition for uncertain terrain is illustrated on the right.}
    \label{fig: uncertainguard}
    \vspace{-2mm}
\end{figure}


\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/motivation_figure.pdf}
    \caption{Demonstration of a periodic orbit with $\max |\lambda(D P(x^*))| < 1$ (illustrated on the left) not being robust to variations in the guard condition (for this example, the ground height was increased by 1cm), while a periodic orbit with a larger $|\lambda|$ (illustrated on the right) is comparatively more robust.}
    \label{fig: motivation}
\end{figure}

\newsec{Motivation}
Practically, the stability of periodic orbits can be analyzed by evaluating the eigenvalues of the Poincar\'e return map linearized around the fixed point. Specifically, if the magnitude of the eigenvalues of $DP(x^*) = \frac{\partial P}{\partial x}(x^*)$ is less than one (i.e. $\max |\lambda (DP(x^*))| < 1$), then the fixed point is stable \cite{perko2013differential,morris2005restricted,wendel2010rank}. 
% Note that in this process, the eigenvalues corresponding to states known to be nonperiodic, such as the horizontal position of the floating base frame. 
Since it is often difficult to compute the Poincar\'e map analytically, it is commonly numerically approximated.  By applying small perturbations to each state and forward simulating one step to obtain $P(x^*+\delta )$ which is then used to construct each row of the Jacobian successively.  This implicitly implies that the Poincar\'e map is robust to $\delta$ perturbations---as long as $\delta$ is sufficiently small.   Yet, this small amount of robustness inherent in stable gaits is often confounded with the eigenvalues themselves.  That is, it is sometimes assumed that the magnitude of the eignevalues of the Poincar\'e map say something deeper about the broader robustness of the periodic orbit to perturbations.  This is not the case, as the following example illustrates. 


    
% \begin{remark}
%     Orbits $\O$ with lower $\lambda_{\max}$ are regarded as being \textit{more stable} than orbits with higher $\lambda_{\max}$ since they are more contractive around the fixed point.
% \end{remark}

% However, since the Poincar\'e map is evaluated at the fixed point, this notion of stability is only valid locally. This means that while this tool is useful for checking the stability of periodic orbits, it is no longer insightful for systems with uncertain guard events or disturbances that push the system away from the fixed point. 

% \subsection{Simulation Example}
% \blue{Take two gaits, with one gait having a smaller eigenvalues than the other. Show that in the presence of uncertain terrain, the "more stable gait" fails, while the other one doesn't.}

\begin{example}
Consider a 5-link bipedal robot shown in Figure \ref{fig: uncertainguard}.  To illustrate how the eigenvalues associated with the linearization fail to tell the whole story, we will consider the robustness of these gaits to differing ground height conditions.  
As illustrated in Figure \ref{fig: motivation}, the classic Poincar\'e analysis does not accurately reflect the robustness of periodic orbits to local disturbances in the guard condition. That is, the gait with the smaller maximum eigenvalue (magnitude) is more fragile to changing ground heights. 
%In this work, we will instead propose tools for discussing the stability of walking (described by either periodic and nonperiodic orbits) from a set-theoretic perspective. This will then allow us to introduce tools for analyzing the stability of walking away from the fixed point.
\end{example}


\newsec{Set-Based Robustness}
% Next, we will extend the notion of set-stable walking to include uncertain guard conditions. 
We now formulate a notion of robustness of the extended Poincar\'e map to uncertain guard conditions. 
Specifically, we consider the general guard (as defined in \cite{hamed2016exponentially}) for some $d \in \R$,
\begin{align}
    S_d &= \{x\in \mathcal{X} \mid h(x) = d, ~\dot h(x) < 0\},
    \label{eq: heightguard}
\end{align}
with $d \in \mathbb{D}$ and $\mathbb{D} := [d^-,d^+] \subset \R$ for some $d^- < 0 < d^+$. Using this general guard definition, the previous guard \eqref{eq: zeroguard} is now denoted as $S_0$.  Under the assumption that $S_d \subset D$ for all $d \in \mathbb{D}$, we have a corresponding hybrid system: 
\begin{numcases}{\mathcal{H}_d  = }
\dot{x} = f_{\rm cl}(x) := f(x) + g(x) k(x) & $x \in D \setminus S_d$, \label{eq: continuousd}
\\
x^+ = \Delta(x^-) & $x^- \in S_d$, \label{eq: discreted}
\end{numcases}

% It is important to note that the typical assumptions made for systems considering $\S_0$ still apply for systems considering $\S_d$ with $d \not= 0$. Mainly,
% \begin{enumerate}
%     \item The continuous-time dynamical system \eqref{eq: continuous} is continuous on $\X$ for any guard condition $S_{d}$
%     \item The solution to \eqref{eq: continuous} from any initial condition $x_0 \in \Delta(S_d)$ is unique and depends continuously on $x_0$ for any guard condition $S_{d}$
%     \item The function $h: \X \to \R$ is differentiable such that for every $s \in S_d$, $\frac{\partial h}{\partial s}(x) \not= 0$ for any $d \in \mathbb{D}$
% \end{enumerate}

Consider the extended time to impact function $T_e : B_{\rho}(x^*) \to \R$ defined implicitly in \eqref{eqn:extendedtimetoimpact}.  This function can be further extended (as a partial function) to account for varying guards: $T_e : B_{\rho}(x^*) \times \mathbb{D} \partialto \R$:
\begin{align}
    T_e(x_0,d) := \inf\{ t \geq 0 \mid \varphi_t(x_0) \in S_d \}.
\end{align}
Importantly, this is a partial function because (by the implicit function theorem) it is only well-defined for $d = 0$ and by continuity sufficiently small $d^-$ and $d^+$.  
Using this extended time-to-impact function, we can define the extended Poincar\'e map as a partial function: $P_d: B_{\rho}(x^*) \partialto S_d$:
\begin{align}
    P_{d}(x^-) := \varphi_{T_e(\Delta(x^-),d)}(\Delta(x^-)).
\end{align}
We now frame robust walking as the forward invariance of this map, for all $d$. 
%Note that the key feature of this definition $\delta$, wherein the goal is to find periodic gaits with maximum $\delta$. 

% The extended time-to-impact function $T_e: \bar{\X} \times \mathbb{D} \to \R^+$ is then defined similarly to the time-to-impact function, with the exception that it is specific to the guard $S_d$:
% \begin{align}
%     T_e(x_0,d) := \inf\{ t \geq 0 \mid \varphi_t(x_0) \in S_d \}.
% \end{align}
% Note here that $T_e$ is well-defined for the neighborhood $\bar{\X}$ satisfying:
% $$\bar{\X} := \{x \in \X \mid 0 < T_e(x,d) < \infty, \dot{h}(x) < 0, \forall d \in \mathbb{D}\}.$$
% Using this extended time-to-impact function, we can define the extended Poincar\'e map, $P_{d}: \bar{S} \to S_d$:
% \begin{align}
%     P_{d}(x^-) := \varphi_{T_e(\Delta(x^-),d)}(\Delta(x^-)),
% \end{align}
% that is well-defined for the open set $\bar{S} := \Delta^{-1}(\bar{X})$.



% Note that this extended Poincar\'e map is well-defined and continuous in a neighborhood around $x_{k-1}$ (\red{can prove in Appendix by extending Lemma 3 in \cite{grizzle2001asymptotically}}). In other words, the Poincar\'e map is defined as $P_{d_k}: \widetilde{S}_{d_{k-1}} \to S_{d_k}$ with $\widetilde{S}_{d_{k-1}} := \Delta^-(\widetilde{\X})$ for $\widetilde{X} := \{x \in \X \mid 0 < T_e(x,d_k) < \infty \}$. 

% Also note that the extended Poincar\'e map for some interval range $d \in [d^-,d^+] \in \R$ can also be interpreted as a set-valued Poincar\'e map:
% \begin{align}
% \P_{[d^-,d^+]}(x):= \{ P_d(x) \mid \forall d \in [d^-,d^+]\}
% \label{eq: setvaluedP}
% \end{align}

% We are now prepared for the following definition:
\begin{definition}  
\label{def: deltarobust}
Let $\O$ be a periodic orbit with fixed point $P_0(x^*) = x^* \in \O \cap S_0$ corresponding to the guard condition $\S_0$ as in \eqref{eq: heightguard}. The orbit $\O$ is \textbf{$\delta$-robust} for a given $\delta > 0$ if:
\begin{align*}
    P_d(\B_{\delta}(x^*)) \subseteq \B_{\delta}(x^*), ~\forall d \in [d^-_{\delta},d^+_{\delta}],
\end{align*}
with the bounds on $d$, $[d^-_{\delta},d^+_{\delta}]$, implicitly determined by: 
$$
d^-_{\delta} = \inf_{x \in B_{\delta}(x^*)} h(x), \qquad 
d^+_{\delta} = \sup_{x \in B_{\delta}(x^*)} h(x).
$$
% Moreover, $\O$ is \textbf{$\delta$-robustly exponentially stable} if there exists an $\epsilon > 0$ such that:
% \begin{align}
%   \forall ~ x \in B_{\delta + \epsilon}(x^*) \backslash B_{\delta}(x^*)  &  \quad \implies \quad  \nonumber\\
%  & \| P^i_d(x) \|_{B_{\delta}(x^*)} \leq M\alpha^i \|x \|_{B_{\delta}(x^*)}, \nonumber
% \end{align}
% % \begin{align}
% %   \forall ~ x  \:\: \mathrm{s.t.}  \:\:  &  0 < \|x \|_{B_{\delta}(x^*)} < \epsilon \quad \implies \quad  \nonumber\\
% %  & \| P^i(x) \|_{B_{\delta}(x^*)} \leq M\alpha^i \|x \|_{B_{\delta}(x^*)}, \nonumber
% % \end{align}
% for $M > 0$ and $\alpha \in (0,1)$. 
% \begin{align*}
%     d^-_{\delta} := \inf\{ h(x) \mid x \in \B_{\delta}(x^*)\}, \\
%     d^+_{\delta} := \sup \{h(x) \mid x \in \B_{\delta}(x^*)\}.
% \end{align*}
\end{definition}


\begin{remark}
Implicit in this definition is that $P_d$ is a well-defined function, not a partial function, on the entire ball $B_{\delta}(x^*)$.  This is clearly not a guaranteed, or even likely, for a given $\delta > 0$.  Hence the key role of $\delta$ in the definition.  As will be seen, the goal will be to determine the largest such $\delta$ for a given periodic orbit.  More generally, this also leads to a synthesis goal: \emph{find periodic orbits that have the largest $\delta$-robustness.}  
\end{remark}


\newsec{Dynamical System Representation}
It is important to note that we can view $\delta$-robustness from the perspective of forward set invariance of $B_{\delta}(x^*)$.  
%
Consider the following discrete-time dynamical system, dependent on a specific guard height $d = h(x)$ (viewed as a control input):
\begin{align}
    \label{eq: discretetime}
    x_{k+1} = P_{d_k}(x_k), \qquad d_k \in [d^-,d^+] \subset \R
\end{align}
for some sequence of $d_k$, $k \in \N_{\geq 0}$, determining the guard height specific to step $k \in \mathbb{Z}^+$ such that $x_{k+1} \in S_{d_k}$.


\begin{lemma}
    \label{lemma:forwadinvariance}
    Consider the discrete-time system \eqref{eq: discretetime}. If $B_{\delta}(x^*)$ is forward invariant: 
    \begin{eqnarray}
    \label{eqn:forwardsetinvariance}
    x_0 \in B_{\delta}(x^*) \quad \implies  \quad 
    x_{k+1} = P_{d_k}(x_k) \in B_{\delta}(x^*) 
    \end{eqnarray}
    for all $x \in \N_{\geq 0}$ and for every sequence $\{d_k\}_{k \in \N_{\geq 0}}$ with $d_k \in [d^-_{\delta},d^+_{\delta}]$, then $\O$ is $\delta$-robust. 
\end{lemma}

\begin{proof}
Assume that $\O$ is not $\delta$-robust.  Then there exists an $x_0 \in B_{\delta}(x^*)$ and a $d_0 \in [d^-_{\delta},d^+_{\delta}]$ such that $P_{d_0}(x_0) \notin B_{\delta}(x^*)$.  This contradicts the implication in \eqref{eqn:forwardsetinvariance}. 
\end{proof}


% \begin{lemma}
%     \label{lemma: recursiveset}
%     Consider the discrete-time system \eqref{eq: discretetime}. If $\forall x_0 \in \B_{\delta}(x^*)$, $P_{d_k}(x_0) \in \B_{\delta}(x^*)$, then $x_{k+1} \in \B_{\delta}(x^*)$, $\forall k \in \mathbb{Z}^+$.
% \end{lemma}

% \begin{proof}
%     The lemma can be proven via recursion. Let $x_1 := P_{d_k}(x_0)$. Applying the set-valued Poincar\'e return map to $x_1$ yields $x_2 := P_{d_k}(x_1)$. Per the assumption, $x_1 \in \B_{\delta}(x^*)$. Therefore, given that $\forall x \in \B_{\delta}(x^*)$, $P_{d_k}(x) \in \B_{\delta}(x^*)$, then since $x_1 \in \B_{\delta}(x^*)$, $x_2 \in \B_{\delta}(x^*)$. Applying this $k \in \mathbb{Z}^+$ times will eventually yield that $x_{k+1} \in \B_{\delta}(x^*)$.
% \end{proof}


\newsec{Connections with Stability}
We note that there are natural connections between $\delta$-robustness and stability.  As the following result shows, every exponentially stable periodic orbit is $\delta$-robust.  The key point is: one does not know the $\delta$ associated with this orbit, hence does not have a quantification of the robustness.  This is the key differentiator between stability and robustness: the ability to quantify the size of perturbations that are allowed.  

\begin{proposition} 
\label{prop:stabiltytorobust}
Let $\O$ be a periodic orbit with a fixed point $x^* \in \S_0$, i.e., $P_0(x^*) = x^*$. If $x^*$ is an exponentially stable equilibrium point of $x_{k+1} = P_0(x_k)$, then there exists a $\delta > 0$, s.t. $\O$ is $\delta$-robust. 
\end{proposition}


\begin{proof}
Following the conditions on exponential stability as defined in Theorem. \ref{def: expstability}, since $\O$ has an exponentially stable equilibrium point, then $\exists \delta' > 0$,  $i \in \mathbb{N}_{\geq 0}$, such that for all $x \in \B_{\delta'}(x^*)$,such that $P_0^i(x) \in \B_{\delta'}(x^*)$.

Similarly to the proof of Theorem 1 in \cite{grizzle2001asymptotically}, there must exist some non-zero interval $t \in [T_e(x,d^+),T_e(x,d^-)]$ with $d^+ > 0$ and $d^- < 0$ during which $\dot{h}(\varphi_t(x)) < 0$. 

Furthermore, we can select $d^+$ and $d^-$ sufficiently small, such that $\{\varphi_{T_e(x,d^+)}(x),\varphi_{T_e(x,d^+)}(x)\} \in \B_{\delta'}(x^*)$. Therefore, $\{P_{d^-}(x),P_{d^+}(x)\} \in \B_{\delta}(x^*)$. 

Next, since $\varphi_t(x_0)$ is unique and depends continuously on $x_0$, and since $P_d(x) = P_0(x)$ for $d = 0$ lies in the interior of the segment $\varphi_t(x)$ for $t \in [T_e(x,d^+),T_e(x,d^-)]$, then again we can choose $d^+$ and $d^-$ sufficiently small such that
$$ \|P_d(x) - P_0\| \leq \max \{\|P_{d^-}(x) - P_0(x)\|,\|P_{d^+}(x) - P_0(x)\| \}.$$

Finally, let $\delta > 0$ be defined as the ball such that:
\begin{align*}
    d^- = \inf\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}, \\
    d^+ = \sup\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}.
\end{align*}
Then for any $d \in [d^-,d^+]$, $P_d(x) \in \B_{\delta}(x^*)$, $\forall x \in \B_{\delta}(x^*)$.
\red{STILL IN PROGRESS...}
\end{proof}

% \begin{proof}
% Following the conditions on exponential stability as defined in Theorem. \ref{def: expstability}, since $\O$ has an exponentially stable equilibrium point, then $\exists \delta' > 0$,  $i \in \mathbb{N}_{\geq 0}$, such that for all $x \in \B_{\delta'}(x^*)$,such that $P_0^i(x) \in \B_{\delta'}(x^*)$.

% Similarly to the proof of Theorem 1 in \cite{grizzle2001asymptotically}, there must exist some non-zero interval $t \in [T_e(x,d^+),T_e(x,d^-)]$ with $d^+ > 0$ and $d^- < 0$ during which $\dot{h}(\varphi_t(x)) < 0$. 

% Furthermore, we can select $d^+$ and $d^-$ sufficiently small, such that $\{\varphi_{T_e(x,d^+)}(x),\varphi_{T_e(x,d^+)}(x)\} \in \B_{\delta'}(x^*)$. Therefore, $\{P_{d^-}(x),P_{d^+}(x)\} \in \B_{\delta}(x^*)$. 

% Next, since $\varphi_t(x_0)$ is unique and depends continuously on $x_0$, and since $P_d(x) = P_0(x)$ for $d = 0$ lies in the interior of the segment $\varphi_t(x)$ for $t \in [T_e(x,d^+),T_e(x,d^-)]$, then again we can choose $d^+$ and $d^-$ sufficiently small such that
% $$ \|P_d(x) - P_0\| \leq \max \{\|P_{d^-}(x) - P_0(x)\|,\|P_{d^+}(x) - P_0(x)\| \}.$$

% Finally, let $\delta > 0$ be defined as the ball such that:
% \begin{align*}
%     d^- = \inf\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}, \\
%     d^+ = \sup\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}.
% \end{align*}
% Then for any $d \in [d^-,d^+]$, $P_d(x) \in \B_{\delta}(x^*)$, $\forall x \in \B_{\delta}(x^*)$.
% \red{STILL IN PROGRESS...}
% \end{proof}

\newsec{Connections with Input-to-state Stability}
Note that beyond simply finding the $\delta$-robustness of a gait, it may be desirable to ensure exponential stability to $B_{\delta}(x^*)$.  This leads to the following definition: 

\begin{definition}
The periodic orbit $\O$ is \textbf{$\delta$-robustly exponentially stable} if it is $\delta$-robust and there exists an open and connected set $W$ with $B_{\delta}(x^*) \subset W $ such that:
\begin{align}
  \forall ~ x_0 \in W   &  \quad \implies \quad  \nonumber\\
 & \| x_k \|_{B_{\delta}(x^*)} \leq M\alpha^k \|x_0 \|_{B_{\delta}(x^*)},  \quad \forall k \in \N_{\geq 0} \nonumber
\end{align}
% \begin{align}
%   \forall ~ x \in B_{\delta + \epsilon}(x^*) \backslash B_{\delta}(x^*)  &  \quad \implies \quad  \nonumber\\
%  & \| P^i_d(x) \|_{B_{\delta}(x^*)} \leq M\alpha^i \|x \|_{B_{\delta}(x^*)}, \nonumber
% \end{align}
for $M > 0$ and $\alpha \in (0,1)$. 
\end{definition}


There are obvious connections with input-to-state stability \cite{jiang2001input}.  In our setting, the discrete time system $x_{k+1} = P_{d_k}(x_k)$ (with $d_k$ viewed as an input) is (exponentially) input to state stable if: 
\begin{eqnarray}
\label{eqn:expiss}
\| x_k \| \leq M\alpha^k \| x_0\|  + \gamma( \max\{-d^-,d^+\} )
\end{eqnarray}
for $k \in \N_{\geq 0}$, $M > 0$, $\alpha \in (0,1)$, and $\gamma$ a class $\K$ function.  \textcolor{red}{In fact, one could alternatively define $\delta$-robustness by saying that $\O$ is $\delta$-robust for a given $\delta > 0$ if $d^- = -\delta$, $d^+ = \delta$ and there exists an open and connected set $W \subset D$ and containing $x^*$ such that:  
$$
\| x_k \| \leq M\alpha^k \| x_0\|  + \delta. 
$$
for $k \in \N_{\geq 0}$, $M > 0$, $\alpha \in (0,1)$.}

Yet in the case of the current definitions, we can establish the following. 

\begin{theorem}
The periodic orbit $\O$ is $\delta$-robustly exponentially stable if and only if the dynamical system in \eqref{eq: discretetime} is exponentially input-to-state stable \eqref{eqn:expiss}.
\end{theorem}

\blue{New definition}
\begin{definition}
    Consider the discrete-time system \eqref{eq: discretetime} with the guard condition $d_k \in \R$ viewed as an input. Given a periodic orbit $\O$ with a fixed point on the nominal guard condition, $x^* = P_0(x^*)$, the orbit $\O$ is $\delta$-robust for a given $\delta > 0$ if there exists some $M > 0$, $\alpha \in (0,1)$, $\varepsilon > 0$ such that for all $x_0 \in \B_{\varepsilon}(x^*)$, 
    $$ \|x_k \| \geq M \alpha^k \|x_0\| + \delta. $$
\end{definition}


==> Old_Sections/UncertainGuard_old.tex <==
\section{A Set Theoretic Perspective on Walking: $\delta$-Robustness}
\label{sec: uncertainguard}

This section provides the key formulation of robustness considered throughout this paper---that of $\delta$-robustness.  The core concept behind this definition is stability in and of itself is not a sufficiently rich concept to capture robustness, since it is purely local.  Thus, we define a set-theoretic notion of robustness leveraging the Poincar\'e map. 



\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/motivation_figure.pdf}
    \caption{Demonstration of a periodic orbit with $\max |\lambda(D P(x^*))| < 1$ (illustrated on the left) not being robust to variations in the guard condition (for this example, the ground height was increased by 1cm), while a periodic orbit with a larger $\lambda_{\max}$ (illustrated on the right) is comparatively more robust.}
    \label{fig: motivation}
\end{figure}

\newsec{Motivation}
Practically, the stability of periodic orbits can be analyzed by evaluating the eigenvalues of the Poincar\'e return map linearized around the fixed point. Specifically, if the magnitude of the eigenvalues of $DP(x^*) = \frac{\partial P}{\partial x}(x^*)$ is less than one (i.e. $\max |\lambda (DP(x^*))| < 1$), then the fixed point is stable \cite{perko2013differential,morris2005restricted,wendel2010rank}. 
% Note that in this process, the eigenvalues corresponding to states known to be nonperiodic, such as the horizontal position of the floating base frame. 
Since it is often difficult to compute the Poincar\'e map analytically, it is commonly numerically approximated.  By applying small perturbations to each state and forward simulating one step to obtain $P(x^*+\delta )$ which is then used to construct each row of the Jacobian successively.  This implicitly implies that the Poincar\'e map is robust to $\delta$ perturbations---as long as $\delta$ is sufficiently small.   Yet, this small amount of robustness inherent in stable gaits is often confounded with the eigenvalues themselves.  That is, it is sometimes assumed that the magnitude of the eignevalues of the Poincar\'e map say something deeper about the broader robustness of the periodic orbit to perturbations.  This is not the case, as the following example illustrates. 


    
% \begin{remark}
%     Orbits $\O$ with lower $\lambda_{\max}$ are regarded as being \textit{more stable} than orbits with higher $\lambda_{\max}$ since they are more contractive around the fixed point.
% \end{remark}

% However, since the Poincar\'e map is evaluated at the fixed point, this notion of stability is only valid locally. This means that while this tool is useful for checking the stability of periodic orbits, it is no longer insightful for systems with uncertain guard events or disturbances that push the system away from the fixed point. 

% \subsection{Simulation Example}
% \blue{Take two gaits, with one gait having a smaller eigenvalues than the other. Show that in the presence of uncertain terrain, the "more stable gait" fails, while the other one doesn't.}

\begin{example}
Consider a 5-link bipedal robot shown in Figure \ref{fig: uncertainguard}.  To illustrate how the eigenvalues associated with the linearization fail to tell the whole story, we will consider the robustness of these gaits to differing ground height conditions.  
As illustrated in Figure \ref{fig: motivation}, the classic Poincar\'e analysis does not accurately reflect the robustness of periodic orbits to local disturbances in the guard condition. That is, the gait with the smaller maximum eigenvalue (magnitude) is more fragile to changing ground heights. 
%In this work, we will instead propose tools for discussing the stability of walking (described by either periodic and nonperiodic orbits) from a set-theoretic perspective. This will then allow us to introduce tools for analyzing the stability of walking away from the fixed point.
\end{example}


\newsec{Set-Based Robustness}
% Next, we will extend the notion of set-stable walking to include uncertain guard conditions. 
We now formulate a notion of robustness of the extended Poincar\'e map to uncertain guard conditions. 
Specifically, we consider the general guard (as defined in \cite{hamed2016exponentially}) for some $d \in \R$,
\begin{align}
    S_d &= \{x\in \mathcal{X} \mid h(x) = d, ~\dot h(x) < 0\},
    \label{eq: heightguard}
\end{align}
with $d \in \mathbb{D}$ and $\mathbb{D} := [d^-,d^+] \subset \R$ for some $d^- < 0 < d^+$. Using this general guard definition, the previous guard \eqref{eq: zeroguard} is now denoted as $S_0$.  Under the assumption that $S_d \subset D$ for all $d \in \mathbb{D}$, we have a corresponding hybrid system: 
\begin{numcases}{\mathcal{H}_d  = }
\dot{x} = f_{\rm cl}(x) := f(x) + g(x) k(x) & $x \in D \setminus S_d$, \label{eq: continuousd}
\\
x^+ = \Delta(x^-) & $x^- \in S_d$, \label{eq: discreted}
\end{numcases}

% It is important to note that the typical assumptions made for systems considering $\S_0$ still apply for systems considering $\S_d$ with $d \not= 0$. Mainly,
% \begin{enumerate}
%     \item The continuous-time dynamical system \eqref{eq: continuous} is continuous on $\X$ for any guard condition $S_{d}$
%     \item The solution to \eqref{eq: continuous} from any initial condition $x_0 \in \Delta(S_d)$ is unique and depends continuously on $x_0$ for any guard condition $S_{d}$
%     \item The function $h: \X \to \R$ is differentiable such that for every $s \in S_d$, $\frac{\partial h}{\partial s}(x) \not= 0$ for any $d \in \mathbb{D}$
% \end{enumerate}

The extended time-to-impact function $T_e: \bar{\X} \times \mathbb{D} \to \R^+$ is then defined similarly to the time-to-impact function, with the exception that it is specific to the guard $S_d$:
\begin{align}
    T_e(x_0,d) := \inf\{ t \geq 0 \mid \varphi_t(x_0) \in S_d \}.
\end{align}
Note here that $T_e$ is well-defined for the neighborhood $\bar{\X}$ satisfying:
$$\bar{\X} := \{x \in \X \mid 0 < T_e(x,d) < \infty, \dot{h}(x) < 0, \forall d \in \mathbb{D}\}.$$
Using this extended time-to-impact function, we can define the extended Poincar\'e map, $P_{d}: \bar{S} \to S_d$:
\begin{align}
    P_{d}(x^-) := \varphi_{T_e(\Delta(x^-),d)}(\Delta(x^-)),
\end{align}
that is well-defined for the open set $\bar{S} := \Delta^{-1}(\bar{X})$.
% Note that this extended Poincar\'e map is well-defined and continuous in a neighborhood around $x_{k-1}$ (\red{can prove in Appendix by extending Lemma 3 in \cite{grizzle2001asymptotically}}). In other words, the Poincar\'e map is defined as $P_{d_k}: \widetilde{S}_{d_{k-1}} \to S_{d_k}$ with $\widetilde{S}_{d_{k-1}} := \Delta^-(\widetilde{\X})$ for $\widetilde{X} := \{x \in \X \mid 0 < T_e(x,d_k) < \infty \}$. 

% Also note that the extended Poincar\'e map for some interval range $d \in [d^-,d^+] \in \R$ can also be interpreted as a set-valued Poincar\'e map:
% \begin{align}
% \P_{[d^-,d^+]}(x):= \{ P_d(x) \mid \forall d \in [d^-,d^+]\}
% \label{eq: setvaluedP}
% \end{align}

% We are now prepared for the following definition:
\begin{definition}  
Let $\O$ be a periodic orbit with fixed point $P_0(x^*) = x^*$ corresponding to the guard condition $\S_0$ as in \eqref{eq: heightguard}. The orbit $\O$ is \textbf{$\delta$-robust} to $d \in [d^-_{\delta},d^+_{\delta}] \in \mathbb{D} \subset \R$ if there exists a $\delta > 0$ such that:
\begin{align*}
    P_d(x) \subseteq \B_{\delta}(x^*), ~\forall d \in [d^-_{\delta},d^+_{\delta}], \forall x \in \B_{\delta}(x^*)
\end{align*}
with the bounds on $d$ implicitly determined by: 
$$
d^-_{\delta} = \inf_{x \in B_{\delta}(x^*)} h(x), \qquad 
d^+_{\delta} = \sup_{x \in B_{\delta}(x^*)} h(x).
$$
% \begin{align*}
%     d^-_{\delta} := \inf\{ h(x) \mid x \in \B_{\delta}(x^*)\}, \\
%     d^+_{\delta} := \sup \{h(x) \mid x \in \B_{\delta}(x^*)\}.
% \end{align*}
\label{def: deltarobust}
\end{definition}

\begin{theorem} 
Let $\O$ be a periodic orbit with a fixed point $x^* \in \S_0$ such that $P_0(x^*) = x^*$. If $x^*$ is an exponentially stable equilibrium point of $x_{k+1} = P_0(x_k)$, then there $\exists \delta > 0$, s.t. $\O$ is $\delta$-robust to $d \in [d^-_{\delta},d^+_{\delta}]$.
\end{theorem}
\begin{proof}
Following the conditions on exponential stability as defined in Theorem. \ref{def: expstability}, since $\O$ has an exponentially stable equilibrium point, then $\exists \delta' > 0$,  $i \in \mathbb{N}_{\geq 0}$, such that for all $x \in \B_{\delta'}(x^*)$,such that $P_0^i(x) \in \B_{\delta'}(x^*)$.

Similarly to the proof of Theorem 1 in \cite{grizzle2001asymptotically}, there must exist some non-zero interval $t \in [T_e(x,d^+),T_e(x,d^-)]$ with $d^+ > 0$ and $d^- < 0$ during which $\dot{h}(\varphi_t(x)) < 0$. 

Furthermore, we can select $d^+$ and $d^-$ sufficiently small, such that $\{\varphi_{T_e(x,d^+)}(x),\varphi_{T_e(x,d^+)}(x)\} \in \B_{\delta'}(x^*)$. Therefore, $\{P_{d^-}(x),P_{d^+}(x)\} \in \B_{\delta}(x^*)$. 

Next, since $\varphi_t(x_0)$ is unique and depends continuously on $x_0$, and since $P_d(x) = P_0(x)$ for $d = 0$ lies in the interior of the segment $\varphi_t(x)$ for $t \in [T_e(x,d^+),T_e(x,d^-)]$, then again we can choose $d^+$ and $d^-$ sufficiently small such that
$$ \|P_d(x) - P_0\| \leq \max \{\|P_{d^-}(x) - P_0(x)\|,\|P_{d^+}(x) - P_0(x)\| \}.$$

Finally, let $\delta > 0$ be defined as the ball such that:
\begin{align*}
    d^- = \inf\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}, \\
    d^+ = \sup\{h(x) \mid \forall x \in \B_{\delta}(x^*)\}.
\end{align*}
Then for any $d \in [d^-,d^+]$, $P_d(x) \in \B_{\delta}(x^*)$, $\forall x \in \B_{\delta}(x^*)$.
\red{STILL IN PROGRESS...}
\end{proof}

\newpage
\subsection{Question: How do we check $\delta$-robustness given $\O$?}

Consider the following discrete-time dynamical system, dependent on a specific guard height:
\begin{align}
    x_{k+1} = P_{d_k}(x_k)
    \label{eq: discretetime}
\end{align}
for some $d_k \in [d^-,d^+] \in \R$ denoting the guard height specific to step $k \in \mathbb{Z}^+$ such that $x_{k+1} \in S_{d_k}$.

\begin{lemma}
    Consider the discrete-time system \eqref{eq: discretetime}. If $\forall x_0 \in \B_{\delta}(x^*)$, $P_{d_k}(x_0) \in \B_{\delta}(x^*)$, then $x_{k+1} \in \B_{\delta}(x^*)$, $\forall k \in \mathbb{Z}^+$.
    \label{lemma: recursiveset}
\end{lemma}
\begin{proof}
    The lemma can be proven via recursion. Let $x_1 := P_{d_k}(x_0)$. Applying the set-valued Poincar\'e return map to $x_1$ yields $x_2 := P_{d_k}(x_1)$. Per the assumption, $x_1 \in \B_{\delta}(x^*)$. Therefore, given that $\forall x \in \B_{\delta}(x^*)$, $P_{d_k}(x) \in \B_{\delta}(x^*)$, then since $x_1 \in \B_{\delta}(x^*)$, $x_2 \in \B_{\delta}(x^*)$. Applying this $k \in \mathbb{Z}^+$ times will eventually yield that $x_{k+1} \in \B_{\delta}(x^*)$.
\end{proof}

Since the specific guard condition $d_k$ assigned to step $k$ is unknown, we will use a set-based Poincar\'e map to denote the collection of Poincar\'e return maps for all guard conditions contained within the set $\B_{\delta}(x^*)$:
\begin{align}
    \P_{\delta}(x) := \{P_d(x) \mid \forall d \in [d^-_{\delta},d^+_{\delta}]\}.
\end{align}
Thus, the discrete-time dynamical system for any guard condition $S_d$ with $d \in [d^-_{\delta},d^+_{\delta}]$ is denoted as the expanding set:
\begin{align}
    \bm{X}_{k+1} := \P_{\delta}(x_k).
    \label{eq: setDiscrete}
\end{align}

Using this set-based notion of a discrete-time dynamical system, we propose the following theorem:
\begin{theorem}
    Consider the discrete-time barrier function, $H_{\delta}: \X \to \R$, defined as $H_{\delta}(x):= \delta^2 - \|x - x^*\|^2 \geq 0$. If the following condition is satisfied: 
    $$\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0), \quad \gamma \in (0,1],$$
    for all $x_0 \in \B_{\delta}(x^*)$, then the periodic orbit $\O$ is $\delta$-robust.
\end{theorem}
\begin{proof}
     Given some $\delta > 0$, with corresponding $\{d^-_{\delta},d^+_{\delta}\} \in \R$ per Definition \ref{def: deltarobust}, then the set $\B_{\delta}(x^*)$ is a 0-superlevel set of the continuously differentiable function $H_{\delta}: \X \to \R$ satisfying: 
    \begin{align*}
        \B_{\delta}(x^*) := \{x \in \X \mid H_{\delta}(x) \geq 0\} \\
        \partial \B_{\delta}(x^*) := \{x \in \X \mid H_{\delta}(x) = 0 \}
    \end{align*}
    
    Per Proposition 4 of \cite{agrawal2017discrete}, the discrete-time system \eqref{eq: discretetime}, for a specific choice of $d_k \in [d^-_{\delta},d^+_{\delta}]$, is forward-set invariant with respect to the set $\B_{\delta}(x^*)$ if $H_{\delta}$ satisfies the following conditions for all $x_0 \in \B_{\delta}(x^*)$:
    \begin{enumerate}
        \item $H_\delta(x_0) \geq 0$,
        \item $H_{\delta}(P_{d_k}(x_k))-H_{\delta}(x_k) \geq -\gamma H_{\delta}(x_k)$, \\$\forall k \in \mathbb{Z}^+$, $0 < \gamma \leq 1$,
    \end{enumerate}
    where the second condition can be rewritten as $H_{\delta}(P_{d_k}(x_k)) \geq (1-\gamma) H_{\delta}(x_k)$.

    Using Lemma \ref{lemma: recursiveset}, $P_{d_k}(x_k) \in \B_{\delta}(x^*)$ for all $k \in \mathbb{Z}^+$ if $P_{d_k}(x_0) \in \B_{\delta}$ for all $x_0 \in \B_{\delta}(x^*)$. Thus, we only need to check the second condition for some set $x_0 \in \B_{\delta}(x^*)$:
    $$H_{\delta}(P_{d_k}(x_0)) \geq (1-\gamma)H_{\delta}(x_0), ~0 < \gamma \leq 1.$$ Lastly, the above condition can be checked for all $d_k \in [d^-_{\delta},d^+_{\delta}]$ by ensuring that the smallest condition $$\min_{d \in \mathbb{D}}\{H_{\delta}(P_{d}(x))\} \geq (1-\gamma)H_\delta(x), $$ is satisfied. 
    Thus, the condition $$\min \{H_{\delta}(\bm{X}_{k})\} \geq (1-\gamma)H_{\delta}(x_0), \quad \gamma \in (0,1],$$ for all $x_0 \in \B_{\delta}(x^*)$ enforces that 
    $\bm{X}_{k+1} = \P_{\delta}(x_k)$ is forward set invariant with respect to the set $\B_{\delta}(x^*)$. This is equivalent to the statement that $ P_d(\B_{\delta}(x^*)) \subseteq \B_{\delta}(x^*), ~\forall d \in [d^-_{\delta},d^+_{\delta}]$. Therefore, per Definition \ref{def: deltarobust}, $\O$ is $\delta$-robust to $d \in [d^-_{\delta},d^+_{\delta}]$.
\end{proof}

% \begin{theorem}
%     If $ H_{\delta}(P_{d_k}(x_k)) \geq \gamma H_{\delta}(x_k)$ for all $x_k \in \B_{\delta}(x^*)$, then $\O$ is $\delta$-robust and the discrete-time system \eqref{eq: discretetime} is exponentially stable.
% \end{theorem}
% \begin{proof}
%     \red{?}
% \end{proof}


% We can use sample-based approach:
% \begin{enumerate}
%     \item Starting with a small $\delta > 0$, fix $\delta > 0$ and sample the boundary of $\B_{\delta}(x^*)$ (i.e. $s_i \sim \partial \B_{\delta}(x^*))$)
%     \item Observe the flow $\varphi_t(\Delta(s_i))$ $\forall s_i \in samples$
%     \item The set-valued Poincar\'e map is equal to a portion of this flow: $$ \P_{[d^-,d^+]}:=\{ \varphi_t(\Delta(s_i)) \mid t \in [T_e(\Delta(s_i),d^+),T_e(\Delta(s_i),d^-)]\}$$ \red{Note: This currently assumes that $\dot{h}<0$ for $h \in [d^-,d^+]$}
%     \item If $\P_{[d^-,d^+]}(s_i) \in \B_{\delta}(x^*)$ for the selected $\delta > 0$, then increase $\delta$ and repeat the process. If not, then the orbit $\O$ is $\delta$-robust to $d \in [d^-,d^+]$.
% \end{enumerate}

\newsubsec{Probablistic Verification Approach}
It is important to recognize that verifying the condition $\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0)$ for all $x_0 \in \B_{\delta}(x^*)$ is computationally infeasible. This is especially true for systems in which the Poincar\'e map is not available explicitly. Thus, we will instead use sampling methods to verify $\delta$-robustness with probabilistic guarantees. 

% Mainly, we will transform the problem into the following uncertain program:
% \begin{align}
%     \delta^* = &\argmax_{\delta > 0} \delta \\
%     &\text{s.t. } H_{\delta}(P_{d_k}(x_k)) \geq H_{\delta}(x_k), ~ 
% \end{align}

As outlined in \cite{akella2022barrier}, the certification of barrier functions can be probabilistic verified using sampling methods. First, we will introduce the method for verifying that a given periodic orbit is $\delta$-robust, for a given $\delta$. This algorithm is provided in Algorithm \ref{alg: givendelta}, and is outlined as follows.

\begin{algorithm}[tb]
\caption{Probabilistic Verification of Lemma 1}\label{alg: givendelta}
\begin{algorithmic}[1]
\Procedure{Given $\delta > 0$}{}
% {$\delta > 0$, $d^-_{\delta} := \inf\{h(x) \mid \B_{\delta}(x^*)\}$, $d^+_{\delta} := \sup\{h(x) \mid \B_{\delta}(x^*)\}$}
\State $x' \sim U(\B_{\delta}(x^*))$
\State Forward simulate $\P_{\delta}(x') \rightarrow \bm{X}_{1}$
\If {$\min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0)$, $0 < \gamma \leq 1$} 
  \State $r_i = 1$
\Else
    \State $r_i = 0$
\EndIf 
\State Repeat sampling $r_i \to \{r_j\}^N_{j=1}$
\State Find minimum $r_j \to r^*_N$
\State Compute $\Prob_{\pi_r}^N[\Prob_{\pi_r}[r \geq r^*_N] \geq 1 - \varepsilon] \geq 1 - (1-\varepsilon)^N$
\EndProcedure
\end{algorithmic}
\end{algorithm}

%%% THIS SECTION NEEDS WORK
-----

Let $r$ be a random variable with an associated probability distribution $\pi_r$. To formalize this distribution, we define the indicator function $\bm{1}_x$


We can as such define the probability of sampling $r$ as the probability of sampling an initial condition $x \in \B_{\delta}(x^*)$ such that the corresponding set-valued Poincar\'e map $\P_{\delta}(x)$ is contained within the set $\B_{\delta}(x^*)$. As stated before, this condition is equivalent to the barrier function condition $\min \{H_{\delta}(\P_{\delta}(x))\} \geq (1-\gamma)H_{\delta}(x)$, for some $0 < \gamma \leq 1$.

In Algorithm \ref{alg: givendelta}, it is assumed that $\delta > 0$ is given. Then, by sampling $x' \in \B_{\delta}(x^*)$ with a uniform distribution over $\B_{\delta}(x^*)$, we can implicitly define the probability distribution function $\pi_r$ for the random variable $r$.

-----

To identify the largest $\delta > 0$ such that $\O$ is $\delta$-robust, consider the following optimization problem
\begin{align}
    \label{eq: optdelta}
    (\delta^*, \gamma^*) = &\argmax_{\delta > 0,\gamma \in (0,1]} \gamma \\
    &\text{s.t. } \min \{H_{\delta}(\bm{X}_{1})\} \geq (1-\gamma)H_{\delta}(x_0) \notag \\
    & \quad \forall x_0 \in \B_{\delta}(x^*) \notag
\end{align}

Again, we can use sampling to probabilistically identify $\delta^*$ and $\gamma^*$ using Algorithm \ref{alg: maxdelta}.

\begin{algorithm}[tb]
\caption{Probabilistic Approach to \eqref{eq: optdelta}}\label{alg: maxdelta}
\begin{algorithmic}[1]
\Procedure{}{}
% {$\delta > 0$, $d^-_{\delta} := \inf\{h(x) \mid \B_{\delta}(x^*)\}$, $d^+_{\delta} := \sup\{h(x) \mid \B_{\delta}(x^*)\}$}
\State $\delta' \sim U(\Omega)$
\State Verify $r^*_N \geq 0$ given $\delta'$ using Alg. \ref{alg: givendelta}
\If {$r^*_N \geq 0$}
    \State Add $\delta'$ to $\{\delta_j\}^N_{j=1}$
\Else
    \State Reject $\delta'$
\EndIf
\State $\max\{\delta_j\}^N_{j=1} \rightarrow \delta^*_N$
\State Compute $\Prob_{\pi_{\delta}}^N[\Prob_{\pi_{\delta}}[\delta \leq \delta^*_N] \geq 1 - \varepsilon] \geq 1 - (1-\varepsilon)^N$
\EndProcedure
\end{algorithmic}
\end{algorithm}


%%%%% OLD STUFF!! 
% \subsection{Theoretical Guarantees using Stochastic Processes}

% The discrete-time dynamical system in the presence of uncertain impact events can be considered as a stochastic system:
% $$ x_{k+1} = P_d$$

% Our definition for Hybrid Set Invariant walking can now be extended to the following:
% \begin{definition} 
%     A hybrid system $\H\C$ with a periodic orbit $\O$ is defined as \textit{Robustly Hybrid Set Invariant} if there exists some set $\D := \{x^-_i \in S \oplus S_d \mid \forall d \in [-\gamma,\gamma]\}$ such that $P_d(x^-_i) \in \D$ for all $x^-_i \in \D$ and for all $d \in [-\gamma, \gamma]$. .
% \end{definition}

% \subsection{Proving that an orbit $\O$ is Robustly HSI}
% Let $H$ denote the trajectory of the guard condition $h(x)$ (in our case the vertical position of the swing foot relative to the stance foot) computed by:
% $$ H(x_0,d) := \{ h(\varphi_t(x_0) \mid 0 \leq t \leq T_{e}(x_0,d)\} \in \R.$$ 

% \begin{assumption}
%     We assume that for $x_0 = \Delta(x^*)$, there exists some $\{T_h,h_{\max}\} \in \R^+$ such that the flow of the system $\varphi_t(x_0)$ evolves such that:
%     \begin{small}
%     \begin{numcases}{}
%         h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) > 0 & $0 \leq t < T_h$, \notag \\
%         h(\varphi_t(x_0)) = h_{\max}, ~\dot{h}(\varphi_t(x_0)) = 0 & $t = T_h$, \notag  \\
%         h(\varphi_t(x_0)) < h_{\max}, ~\dot{h}(\varphi_t(x_0)) < 0 & $T_h < t < T_e(x_0,-\gamma)$, \notag \\
%         h(\varphi_t(x_0)) = -\gamma, ~\dot{h}(\varphi_t(x_0)) < 0 & $t = T_e(x_0,-\gamma)$. \notag
%     \end{numcases}
%     \end{small}
%     \label{assump: swingfoot}
% \end{assumption}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/swingfoot.pdf}
%     \caption{Example Swing Foot Trajectory Satisfying Assumption \ref{assump: swingfoot}.}
%     \label{fig: swingfootassump}
% \end{figure}

% \begin{lemma}
%     Let $H(x_0,-\gamma)$ be a trajectory of the continuous guard condition $h(x) \in \R$ that satisfies Assumption \ref{assump: swingfoot}. If $h_{\max} \geq \gamma$, then %if $h(\varphi_t(\Delta(x^*))) \in \R^+$ is monotonically decreasing for all $t \in [T_h, T_e(x_0,-\gamma)]$, and  then 
%     $$T_e(\Delta(x^*),\gamma) \leq T_e(\Delta(x^*),0) \leq T_e(\Delta(x^*),-\gamma).$$ 
%     \label{lemma: orderedtime}
% \end{lemma}
% \begin{proof}
%     Per assumption \ref{assump: swingfoot}, the evaluation of the guard condition is $h(\varphi_t(x_0)) = \{h_{\max},-\gamma\}$ for $t = \{T_h, T_e(x_0,-\gamma)\}$. Additionally, we know that $h(\varphi_t(x_0))$ is monotonically decreasing in the interval $t \in (T_h,T_e(x_0,-\gamma))$ due to the assumption that in this range, $\dot{h}(\varphi_t(x_0)) < 0$. Thus, by the intermediate value theorem, we know that there must exist some $\{T_e(x_0,\gamma),T_e(x_0,0)\} \in (T_h,T_e(x_0,-\gamma))$ such that $\{h(\varphi_{T_e(x_0,0)}(x_0)),h(\varphi_{T_e(x_0,\gamma)}(x_0)) \} \in (h(\varphi_{T_h}(x_0)), h(\varphi_{T_e(x_0,-\gamma)}(x_0)))$. Additionally, since $h$ is monotonically decreasing in $t \in (T_h,T_e(x_0,-\gamma))$, then $h(\varphi_t(x_0)) = \gamma$ will occur at time $T_e(x_0,\gamma)$ before the height will reach $h(\varphi_t(x_0)) = 0$ at time $T_e(x_0,0)$. Thus, $T_e(x_0,\gamma) \leq T_e(x_0,0) \leq T_e(\Delta(x^*),-\gamma)$. 
% \end{proof}

% For ease of notation, we will denote the flow of our system between the guards $S_{\gamma}$ and $S_{-\gamma}$ as:
% \begin{align}
%     \varphi^*_t(x_0) := \{ \varphi_t(x_0) \mid T_e(x_0,\gamma) \leq t \leq T_e(x_0,-\gamma) \}.
% \end{align}
% \begin{lemma}
%     Consider a periodic orbit $\O$ with a fixed point $x^* \in \S_0$ satisfying $P_{0,0}(x^*) = x^*$. Assuming that $H(x_0,-\gamma)$ satisfies the properties of Assumption \ref{assump: swingfoot} for $x_0 = \Delta(x^*)$ and enforcing $h_{\max} \geq \gamma$, then the following holds:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmax_{t \in R^+} \|\varphi^*_t(x_0) - x^*\|
%     \end{align}
% \end{lemma}
% \begin{proof}
% It is known that $h: \X \to \R$ is continuous with $\dot{h} < 0$ for $t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)]$. It is also known that the arguments of $h$ (i.e. $\varphi_t(x_0) \in \X$) are also continuous. Thus, since $\|\varphi^*_t(x_0) - x^*\| = 0$ lies in the interior of $t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)]$ (using the ordering of $T_e(x_0,\gamma) \leq T_e(x_0,0) \leq T_e(\Delta(x^*),-\gamma)$ from Lemma \ref{lemma: orderedtime}), then $h(x)$ must take its largest values at the boundary of the set ($t =\{T_e(x_0,\gamma),T_e(x_0,-\gamma)\}$).
% \end{proof}

% \red{Next, we will assume that the continuous-time flow of some periodic orbit $\O$ satisfies the following assumption. Note that we later prove that this assumption is true for certain bipedal systems.}
% \begin{assumption}
%     Assume that given a periodic orbit $\O$ with a fixed point $P_0(x^*) = x^*$, then $\varphi^*(\Delta(x^*))$ evolves such that for $x_0 := \Delta(x^*) \in \Delta(\S_0)$:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmax_{t \in R^+} \|\Delta(\varphi^*_t(x_0)) - \Delta(x^*)\|
%     \end{align}
%     \label{assumption: maxTreset}
% \end{assumption}

% \begin{lemma}
%     (For systems with one degree of underactuation) If the following is true: 
%     $$\{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmin_{t \in R^+} \|\Delta(\varphi^*_t(x_0)) - \Delta(x^*)\|, $$
%     then the following is also true:
%     \begin{align}
%         \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\} = \argmin_{t \in R^+} \|P_{i}(\varphi^*_t(x_0)) - x^*\|, \notag \\
%         ~\forall i \in [-\gamma, \gamma]
%     \end{align}
%     \label{lemma: maxTpointcare}
% \end{lemma}
% \begin{proof}
%     \red{? Need to make an argument about the flow $\varphi_t(x_0)$.... I think this also relies on the assumption that you have only one degree of underactuation plus some assumption about your closed loop system (maybe an ISS assumption about $\O$)}
% \end{proof}

% \begin{theorem}
%     Let $\O := \{\varphi_t(\Delta(x^*)) \mid 0 \leq t \leq T_e(\Delta(x^*),0) \}$ be a periodic orbit with a fixed point $x^*\in\S_0$ such that $P_{0,0}(x^*) = x^*$. Also, assume that $H(\Delta(x^*),-\gamma)$ satisfies Assumption \ref{assump: swingfoot}. Denote an early and late impact state associated with the flow $\varphi_t(\Delta(x^*))$ as:
%     \begin{align*}
%         x_e &:= \{\varphi_t(\Delta(x^*)) \in \X \mid t = T_e(\Delta(x^*),\gamma)\}, \\
%         x_l &:= \{\varphi_t(\Delta(x^*)) \in \X \mid t = T_e(\Delta(x^*),-\gamma)\}.
%     \end{align*}
%     Additionally, denote the Poincar\'e return map associated with the Poincar\'e sections $S_{\gamma}$ and $S_{-\gamma}$ as:
%     \begin{align*}
%         P_e(x) := \{ \varphi_{t}(\Delta(x)) \mid t = T_e(\Delta(x),\gamma) \}, \\
%         P_l(x) := \{ \varphi_{t}(\Delta(x)) \mid t = T_e(\Delta(x),-\gamma) \}
%     \end{align*}
%     The orbit $\O$ is \textit{Robustly Hybrid Set Invariant} for the set $\D := \textup{conv}(\{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\})$ if:
%     \begin{align*}
%         \varphi_t(x_0) \in \D, ~&\forall t \in [T_e(x_0,\gamma),T_e(x_0,-\gamma)], \\
%         &\forall x_0 \in \{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\}
%     \end{align*}
% \end{theorem}
% \begin{proof}
%     For $\D := \textup{conv}(\{P_e(x_e),P_e(x_l),P_l(x_e),P_l(x_l)\})$, the orbit $\O$ is Robustly HSI if $P_d(x^-_i) \in \D$ for all $d \in [-\gamma,\gamma]$ and for all $x^-_i \in \D$.
%     Following Lemma \ref{lemma: maxTpointcare}, we know that the Poincar\'e map error is maximized for the flow $\varphi_t(x_0)$ evaluated at $t = \{T_e(x_0,\gamma),T_e(x_0,-\gamma)\}$. Thus, it suffices to check the Poincar\'e return map of $x_e$ and $x_l$....
%     By ensuring that the flow $\varphi^*_t(x_0)$ remains within the convex hull of $\D$, then any point within the convex set must also return to $\D$. Thus, $P_d(\D) \in \D$ for any $d \in [-\gamma, \gamma]$.
%     % Furthermore, these pre-impact states will yield the largest subsequent error for the set of states $\D := \{P_e(x_e),P_e(x_l), P_l(x_e), P_l(x_l)\}$. Finally, 
% \end{proof}


==> Old_Sections/WalkingSection.tex <==
\newpage
\section{Connections with Walking}
The set-based definitions of walking can be specialized for the specific application of legged locomotion. Inspired from Definition 1 of \cite{ames2015first}, we can define the set of hybrid flows $\{\C,\D\}$ as a \textit{walking gait} using the following definition. Notably, this definition of walking includes but is not limited to periodic orbits. 
\begin{definition}
A collection of hybrid flows $\{\C, \D\}$ is defined as a \textit{walking gait} if there exist constants $T_{I}^{\text{min}} > 0$ and $p_{com}^{\text{min}} > 0$ such that for every element $x^-_i \in \D$:
% with the corresponding hybrid flow $\C_i \in \C$, 
\begin{align}
    T_I(x^-_i) > T_{I}^{\text{min}}, \tag{Non-Zeno Behavior} \\
    \dot{p}_{\com}^x(P(x^-_i)) > 0, \tag{Progress} \\
    \min_{t \in \leq T_I(x^-_i)} p_{\com}^y(\varphi_t(\Delta(x^-_i))) > p_{\com}^{\min}, \tag{Upright} \\
    % P(\D^i) = \D_{i+1}. \tag{Continuity}
\end{align}
\label{def: walkinggait}
\end{definition}

While Definition \ref{def: walkinggait} provides us with a set-based perspective of walking, we do not yet have constructive tools for how to enforce such set-based walking gaits. To this end, we propose the following theorem,

\begin{theorem}
    Assume there exists a set $\D$ such that $P(\D) \subset \D$, then the conditions listed in Def. \ref{def: walkinggait} are satisfied for all $x_0 \in \D$.
\end{theorem}
\begin{proof}
    \red{Prove this by construction with barrier functions.}
\end{proof}

\begin{corollary}
    When enforced, the following three barrier functions result in set-based stable walking.
    \begin{align}
        h_1 &:= \tau_{i+1}-\tau_{i}-\tau_{\text{min}} \tag{Barrier for Dwell Time} \\
        h_2 &:= \dot{p}_{\text{com}}^x(x_i(\tau_{i+1})) \tag{Barrier for Progress} \\
        h_3 &:= p_{\com}^y(x_i(t)) - p_{\com}^{\min} \tag{Barrier for Upright}
    \end{align}
\end{corollary}

\begin{comment}
\subsection{Enforcing Set-Based Stability}
Although we now have set-based definitions of discrete-time stability for systems with impulse effects, we do not yet have constructive tools for enforcing this stability, or even checking whether a system has a set $\D$ such that $P(\D) \subset \D$. 

One method towards enforcing set-based stability is via  barrier functions.

One method of checking whether a system is set-based stable is via sampling.
\end{comment}
